Are Vision Transformers Robust to Spurious Correlations?

Deep neural networks may be susceptible to learning spurious correlations that hold on average but not in atypical test samples. As with the recent emergence of vision transformer (ViT) models, it remains underexplored how spurious correlations are manifested in such architectures. In this paper, we systematically investigate the robustness of vision transformers to spurious correlations on three challenging benchmark datasets and compare their performance with popular CNNs. Our study reveals that when pre-trained on a sufficiently large dataset, ViT models are more robust to spurious correlations than CNNs. Key to their success is the ability to generalize better from the examples where spurious correlations do not hold. Further, we perform extensive ablations and experiments to understand the role of the self-attention mechanism in providing robustness under spuriously correlated environments. We hope that our work will inspire future research on further understanding the robustness of ViT models.

==> section/domain_invariant.tex <==
\section{Training with different domain invariant objectives}
\label{sec:domain_invariant}

In recent literature, many works have been proposed to tackle the issue of domain generalization, which mainly focuses to achieve high classification accuracy on new test environments consisting of inputs with invariant features. Sagawa \textit{et al.}~\cite{sagawa2019distributionally} has shown that significant improvement can be achieved in worst-group test accuracy by training CNNs using group Distributionally Robust Optimization(GDRO). In this section, we investigate if training ViT models with domain invariant objectives can further increase their robustness to spurious correlations.

\vspace{0.2cm}
\noindent \textbf{Takeaways} Table \ref{tab:domain_invariant} reports evaluation results for ViT models of different capacities when fine-tuned on Waterbirds dataset using ERM and GDRO. We observe...

\input{tables/domain_invariance_table}

==> section/experiments.tex <==

\section{Experiments}
\label{sec:exp}

\subsection{ColorMNIST} 
    It is a modified version of MNIST~\cite{mnist}, where the digits are superimposed on coloured backgrounds. Similar to the setup in~\cite{ming2021impact}, while training the model, we fix the in-distribution classes $\mathcal{Y}$ as $\{0,1\}$ and the background colors $\mathcal{E}$ as $\{red, green, purple, pink\}$. Note, while training the foreground color is same as in MNIST~\cite{mnist} ,i.e., $\texttt{white}$. The correlation ratio $r$, defined as P(e = red | y = 0) = P(e = purple | y = 0) = P(e = green | y = 1) = P(e = pink | y = 1), is set from $\{0.25,0.35,0.45\}$ for this paper. In this case, the spurious features include background and foreground color, whereas the invariant features constitutes the digit shape.\\
\textbf{Spurious Correlation Testing setup : }To investigate the robustness of various models under spuriously correlated environments, we define a new setup ( as in figure below) by changing the color of both the background and foreground digit. Ideally, the predictions of a robust model should not be correlated with the change in the spurious features, which are background and foreground colors and only depend on shape of the digit ,i.e., the invariant feature. Specifically, we come up with the following three strategies :

\begin{enumerate}
    \item \textbf{Measuring Accuracy :} In this step, we aim to measure the dependence of various models on spurious features while making predictions. To meet that end, we generate pair of images with same foreground digit but different foreground and background color combinations. Since, we keep the invariant features,i.e, the semantics of the digit same in a pair, a model accurately identifying the classes of both the images can be labelled as more robust, since such a model would have lesser dependence on spurious features while making predictions. Although, we select the foreground and background color randomly, after extensive experimentation we found the setting the foreground color as $\texttt{black}$ and background color as $\texttt{white}$ causes the deep neural models to make most mistakes. Hence, in the rest of the paper, we continue with the same setup.
    
    \item \textbf{Measuring CKA Similarity :} As defined earlier, CKA similarity can be used to measure the notion of similarity between the representations of various layers in a neural net. The main aim or goal of this setup, is to study how much the internal representations of a neural net varies with a change in the spurious features. If altering the spurious features causes a significant change in the feature vectors of network, then it would clearly indicate the model's reliance on spurious features while making predictions. To study this, we first generate a set of images exactly similar to training data in terms of the digit semantics but with an altered background and foreground color. 
    
    Algorithm 1 provides a more detailed understanding of how we calculate the CKA similarity score for a given layer($l$) and neural network($F$). First of all, a mini-batch is sampled from both the training data and the newly curated dataset. Secondly, the representations for layer $l$ are obtained by passing the images through the model. Next, we calculate the CKA similarity between the representations obtained for the two set of images. A higher CKA Similarity score for a network implies lesser dependence on spurious features and more reliable predictions.
   % \input{section/cka_pseudocode}
\end{enumerate}


Furthermore, for spurious OOD we use the digits $\{5,6,7,8\}$ with background color red and green, which contains overlapping spurious features with the training data. For non-spurious OOD, we use the common set of datasets used in past literature such as Textures, LSUN, etc.

\subsection{Waterbirds}
In this dataset, the class label( bird type) is spuriously correlated with the background features. Similar to the setup introduced  in~\cite{sagawa2019distributionally}, we define the in-distribution classes $\mathcal{Y}$ as $\{$waterbird, landbird$\}$. The dataset is formed by selecting bird photographs from the Caltech-UCSD Birds-200-2011 (CUB)~\cite{WahCUB_200_2011} dataset  and then superimposing on either of $\mathcal{E}$ = \{waterbackground, landbackground\} selected from the Places~\cite{zhou2020deep} dataset. The spurious correlation is injected by pairing waterbirds with waterbackground and landbirds with landbackgroud more frequently, as compared to other combinations. Fixing the correlation coefficient,$r = 0.95$, results in the worst or smallest group ,i.e., waterbird on land background to contain 56 training examples out of 4957 total images. \\
\textbf{Testing setup : } To understand the dependence of various deep learning models on using background features while making predictions, we setup the following experiments :

\begin{enumerate}
    \item \textbf{Measuring Accuracy :} Since, in this setup we aim to study the variation in accuracy of a model with the change in spurious features, first a foreground bird photograph is selected from the Caltech-UCSD Birds-200-2011 (CUB) dataset, then the same image is placed on top of a water and land background selected from the Places dataset.  In this way, a pair of images are generated with the same foreground object,i.e., bird type in this case but different background features. Hence, a model which has high reliance on spurious or environmental features, would predict different class labels for each image in a pair indicating its lack of robustness. Similarly, an accurate model would predict same class labels for both images in a pair as they contain exactly similar foreground object. Since, in a pair both the images share the same invariant features (class label), but different environmental features (background), this setup can easily help in identifying models with high reliance on spurious features. We repeat the same process to generate multiple pairs such that each pair has the same foreground object but different background, and report the mean accuracy for each model. 
    
    \item \textbf{Measuring CKA Similarity :} Similar to the previous setup, in this case also we generate multiple pair of images with each pair containing the same foreground bird photograph but different background. Since internal representations of a neural net play vital role in understanding the behaviour of a model under spuriously correlated environments, in this study we calculate the CKA similarity score between images of a bird on a water background and land background for a given layer. A high similarity score would indicate the models robustness against spurious features and vice-versa. 
\end{enumerate}



    
    




==> section/intro.tex <==
\section{Introduction}
\label{sec:intro}
Convolutional neural networks (CNNs)~\cite{He2016DeepRecognition,Krizhevsky2012ImageNetNetworks, Kolesnikov2020BigLearning} has been the main ingredient for the successes of deep learning in visual tasks over the past several years. The key reason of their ubiquitousness is mainly attributed to the ability to encode informative general purpose feature representations through convolutional layers. Based on the powerful inductive bias of translational equivariance and spatial locality, convolutional layers have been an essential part of almost every model deep neural network designed for vision related tasks, and hence been studied extensively~\cite{battaglia2018relational, szegedy2013intriguing, girshick2015deformable} over the past decades. 

Recently, after the unprecedented success of transformer in natural language processing, there has been a deluge of studies adopting the attention-based transformer architecture for various domains such as computer vision. Since the introduction of Vision Transformers(ViT) by Dosovitskiy \textit{et al.}~\cite{dosovitskiy2020image}, the vision community has seen a paradigm shift in state-of-art results on image classification tasks at large scale. Dosovitskiy \textit{et al.}~\cite{dosovitskiy2020image} has shown that when trained on sufficiently large datasets, ViT achieves superior performance as compared to the state-of-art residual networks (ResNets)~\cite{He2016DeepRecognition}. Instead of relying on convolutions, ViT uses multi-head self-attention layers to learn and aggregate meaningful information across various spatial locations. Since after coming to the limelight, ViT models have been widely studied to understand the working principle of various components of the architecture~\cite{raghu2021vision}
, robustness to adversarial \& natural perturbations and distributional shifts ~\cite{naseer2021intriguing, zhang2021delving, paul2021vision, bhojanapalli2021understanding, aldahdooh2021reveal}.\\ 
Machine learning models, are typically trained to generalize better when the test samples are independent and identically distributed (\iid) with the training distribution i.e., test and training samples are drawn from a same stationary distribution~\cite{simonyan2014very}. Previous studies~\cite{hovy2015tagging, tatman2017gender, duchi2019distributionally} have shown that models attaining high accuracy on test set, can still behave inconsistently on rare and untypical examples. One possible reason has been identified as the models reliance on spurious correlations: prediction rules which exist for majority of training examples but do not hold in general. Further, recently~\cite{sagawa2019distributionally} has shown that CNNs when trained on datasets containing spurious correlations, although achieves high test accuracy on average but fails significantly when tested against samples where such correlations do not hold in general. To mitigate this problem,~\cite{sagawa2019distributionally} proposes to use distributionally robust optimization which aims to minimize the worst-case expected loss over the training dataset unlike Empirical Risk Minimization, thereby aiming to reduce the reliance of the model on spurious features while making predictions. Motivated by the setup in ~\cite{sagawa2019distributionally},~\cite{ming2021impact} introduced a novel definition of out-of-distribution(OOD), involving test samples which contain environmental or spurious features but lacks the presence of invariant features, tricking the model to classify these samples as in-distribution(ID). ~\cite{ming2021impact} classify such test samples under the category of Spurious OOD, and experimentally shows the brittleness of modern state-of-art OOD detection methods against such Spurious OOD samples.\\
Recent studies in domain of natural language processing have shown that large pre-trained language models such as BERT excel in improving robustness to spurious correlations. The key reason of success is attributed to the ability of pre-trained models to generalize better from the minority group examples, where spurious correlations do not hold, while finetuning. Intrigued by the fact that pre-training improve robustness to spurious correlations in language-related tasks, in this paper we try to answer the questions :a) First, how does large scale pre-training helps in improving robustness to spurious correlation for image classification tasks. b) Are Vision Transformers more robust to spurious correlations as compared to CNNs. 
\begin{figure}[t]
\centerline{\includegraphics[scale = 0.38]{images/problem_setup.pdf}}
\caption{}
\label{fig:latent_pattern}
\end{figure}









==> tables/celeba_ood_eval.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{15pt}
\begin{table}[h!]
\centering
 \begin{tabular}{l|c|c?c|c}
 \hlineB{2.5}
 \multirow{2}{0.75cm}{\centering Model} & \multicolumn{2}{c}{Spurious OOD} & \multicolumn{2}{c}{Non-spurious OOD} \\
 \cline{2-5}
 & FPR95$\pmb{\downarrow}$ & AUROC$\pmb{\uparrow}$ & FPR95$\pmb{\downarrow}$ & AUROC$\pmb{\uparrow}$ \\
  \hline
 ViT-B/16 & 56.8 & 91.0 & 0 & 0 \\
 \hline
 ViT-S/16 & 61.3 & 86.8 & 0 & 0 \\ 
 \hline
 ViT-Ti/16 & 94.3 & 72.7 & 0 & 0 \\ 
 \hline
 BiT-M-R50x3 & 63.8 & 85.3 & 0 & 0 \\
 \hline
 BiT-M-R101x1 & 70.3 & 85.6 & 0 & 0 \\ 
 \hline
BiT-M-R50x1 & 69.4 & 84.7 & 0 & 0 \\ 
\hlineB{2.5}
 \end{tabular}
 \vspace{0.25cm}
\caption{OOD detection performance of various models when finetuned on CelebA~\cite{liu2015deep}. For Non-spurious OOD, the results are averaged over the test sets of SVHN~\cite{netzer2011reading}, LSUN~\cite{yu2015lsun} and iSUN~\cite{xu2015turkergaze}.}
\label{}

\end{table}


==> tables/cmnist_avg_acc.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.25}
\begin{table}[h!]
\centering
 \begin{tabular}{l|c|c?c|c}
 %\hlineB{2.5}
 
 \hlineB{2.5}
 \multirow{2}{0.75cm}{\centering Model} & \multicolumn{2}{c}{Train} & \multicolumn{2}{c}{Test} \\
 \cline{2-5}
 & Average Acc. & Worst-Group Acc. & Average Acc. & Worst-Group Acc. \\
  \hline
 ViT-B/16 & 100 & 100 & \textbf{96.8} & \textbf{85.3} \\
 \hline
 ViT-S/16 & 100 & 100 & 95.7 & 80.7 \\ 
 \hline
 ViT-T/16 & 95.7 & 44.4 & 86.7 & 28.8 \\ 
 \hline
 BiT-M-R50x1 & 100 & 100 & 92.1 & 74.5 \\ 
 \hline
BiT-M-R101x1 & 100 & 100 & 94.0 & 77.9 \\ 
 \hline
 BiT-M-R50x3 & 100 & 100 & 94.9 & 80.5 \\ 
 \hlineB{2.5}
 \end{tabular}
 \vspace{0.25cm}
\caption{Average and Worst-Group accuracies over train and test set for different models when finetuned on CelebA~\cite{liu2015deep}. Both ViT-B/16 and ViT-S/16 attain better worst-group accuracy as compared to ResNet-V2 based BiT models. }
\label{}
\end{table}

==> tables/cmnist_ood_eval.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{15pt}
\begin{table}[h!]
\centering
 \begin{tabular}{l|c|c?c|c}
 \hlineB{2.5}
 \multirow{2}{0.75cm}{\centering Model} & \multicolumn{2}{c}{Spurious OOD} & \multicolumn{2}{c}{Non-spurious OOD} \\
 \cline{2-5}
 & FPR95$\pmb{\downarrow}$ & AUROC$\pmb{\uparrow}$ & FPR95$\pmb{\downarrow}$ & AUROC$\pmb{\uparrow}$ \\
  \hline
 ViT-B/16 & 56.8 & 91.0 & 0 & 0 & 7.4 & 98.8 \\
 \hline
 ViT-S/16 & 62.2 & 87.0 & 61.3 & 86.7 & 8.7 & 97.7 \\ 
 \hline
 ViT-T/16 & 79.5 & 71.6 & 94.3 & 72.7 & 0 & 0 \\ 
 \hline
 BiT-M-R50x3 & 96.0 & 59.0 & 63.8 & 85.3 & 45.9 & 84.1 \\ 
 \hline
BiT-M-R101x1 & 95.5 & 59.5 & 70.3 & 85.6 & 44.5 & 81.4 \\ 
 \hline
 BiT-M-R50x1 & 95.1 & 63.4 & 69.7 & 85.7 & 30.0 & 88.4 \\ 
 \hlineB{2.5}
 \end{tabular}
 \vspace{0.25cm}
\caption{OOD detection performance of various models when finetuned on Waterbirds~\cite{sagawa2019distributionally}. For Non-spurious OOD, the results are averaged over the test sets of SVHN~\cite{netzer2011reading}, LSUN~\cite{yu2015lsun} and iSUN~\cite{xu2015turkergaze}.}
\label{}
\end{table}


==> tables/domain_invariance_table.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{2pt}
\begin{table}[h!]
\centering
 \resizebox{1\textwidth}{!}{
 \begin{tabular}{l|c|c?c|c?c|c?c|c}
 \hlineB{2.5}
 \multirow{3}{0.75cm}{\centering Model} & \multicolumn{4}{c?}{ERM} & \multicolumn{4}{c}{GDRO}  \\
 \cline{2-9}
 & \multicolumn{2}{c?}{Train} & \multicolumn{2}{c?}{Test} & \multicolumn{2}{c?}{Train} & \multicolumn{2}{c}{Test} \\
\cline{2-9}
 & Average Acc.  & Worst-Group Acc. & Average Acc. &  Worst-Group Acc. & Average Acc. & Worst-Group Acc. & Average Acc. & Worst-Group Acc. \\
  \hline
ViT-B/16 & \textbf{56.8} & \textbf{91.0} & \textbf{60.5} & \textbf{88.4} & \textbf{7.4} & \textbf{98.8} & 85 & 86 \\
 \hlineB{2.5}
 \end{tabular}}
 \vspace{0.25cm}
\caption{\small\textbf{Domain Invariance Training.} Evaluation results of ViT models of different capacities when fine-tuned on Waterbirds~\cite{sagawa2019distributionally}, using ERM and GDRO. \soumya{Currently the numbers in the table are not updated.}}
\label{tab:domain_invariant}
\vspace{-0.8cm}
\end{table}

==> tables/domain_invariance_table_waterbirds.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.25}
\begin{table}[ht]
\centering
\resizebox{0.8\textwidth}{!}{
 \begin{tabular}{l|c|c?c|c}
 %\hlineB{2.5}
 
 \hlineB{2.5}
 \multirow{2}{0.75cm}{\centering Model} & \multicolumn{2}{c}{Train} & \multicolumn{2}{c}{Test} \\
 \cline{2-5}
 & Average Acc. & Worst-Group Acc. & Average Acc. & Worst-Group Acc. \\
\hline
 ViT-B/16 & 76.81 & 0.01 &  77.87 & 0.0 \\

 ViT-S/16 & 97.8 & 87.0 & 95.1 & 86.0 \\ 

 ViT-Ti/16 & 93.2 & 90.8 & 90.7 & 74.3 \\ 

 \hlineB{2.5}
 \end{tabular}}
 \vspace{0.1cm}
\caption{\small Average and worst-group accuracies over train and test set for different models when finetuned on Waterbirds~\cite{sagawa2019distributionally} using GDRO.}
\label{tab:gdro}
\end{table}

\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.25}
\begin{table}[t]
\centering
\resizebox{0.98\linewidth}{!}{
 \begin{tabular}{l|c|c?c|c}
 %\hlineB{2.5}
 
 \hlineB{2.5}
 \multirow{2}{0.75cm}{\centering Model} & \multicolumn{2}{c}{Train} & \multicolumn{2}{c}{Test} \\
 \cline{2-5}
 & Average Acc. & Worst-Group Acc. & Average Acc. & Worst-Group Acc. \\
\hline
 ViT-B/16 & 100 & 100 & 96.9 & 92.0 \\

 ViT-S/16 & 100 & 100 & 93.1 & 82.8 \\ 

 ViT-Ti/16 & 94.0 & 58.8 & 86.8 & 35.8 \\ 
%  \hlineB{2}
%  BiT-M-R50x3 & 100 & 100 & 96.4 & 82.1 \\ 

% BiT-M-R101x1 & 100 & 100 & 96.9 & 83.9 \\ 

%  BiT-M-R50x1 & 100 & 100 & 95.4 & 80.6 \\
 \hlineB{2.5}
 \end{tabular}}
 \vspace{0.1cm}
\caption{\small Average and worst-group accuracies over train and test set for different models when fine-tuned on Waterbirds~\cite{sagawa2019distributionally} using Risk Extrapolation (REx)~\cite{krueger2021out}.}
\label{tab:rex}
\end{table}


==> tables/resnet_scratch.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\renewcommand{\arraystretch}{1.25}
\begin{table}[h]
\centering
 \begin{tabular}{l|c|c?c|c}
 \hlineB{2.5}
 \multirow{2}{0.75cm}{\centering Dataset} & \multicolumn{2}{c}{Train} & \multicolumn{2}{c}{Test} \\
 \cline{2-5}
 & Average Acc. & Worst-Group Acc. & Average Acc. & Worst-Group Acc. \\
\hline
 Waterbirds & 98.0 & 88.0 & 69.1 & 0.07 \\

 CelebA & 100 & 100 & 69.1 & 0.07 \\ 

 CMNIST & & & & \\\
 \hlineB{2.5}
 \end{tabular}
 \vspace{0.1cm}
\caption{\small Average and worst-group accuracies over train and test set for ResNet18 when trained from scratch on Waterbirds~\cite{sagawa2019distributionally}, CelebA~\cite{liu2015deep} and CMNIST.}
\label{tab:resnet_scratch}
\end{table}
